LayoutLLM: Large Language Model Instruction Tuning for Visually Rich Document Understanding

This paper proposes LayoutLLM, a more flexible document analysis method for understanding imaged documents. Visually Rich Document Understanding tasks, such as document image classification and information extraction, have gained significant attention due to their importance. Existing methods have been developed to enhance document comprehension by incorporating pre-training awareness of images, text, and layout structure. However, these methods require fine-tuning for each task and dataset, and the models are expensive to train and operate. To overcome this limitation, we propose a new LayoutLLM that integrates these with large-scale language models (LLMs). By leveraging the strengths of existing research in document image understanding and LLMs' superior language understanding capabilities, the proposed model, fine-tuned with multimodal instruction datasets, performs an understanding of document images in a single model. Our experiments demonstrate improvement over the baseline model in various document analysis tasks.

==> files/abstract.tex <==
Our paper introduces LayoutLLM, a more efficient method for document analysis that involves extracting information and processing imaged documents automatically. 
This technique has gained significant attention in recent years.
Previously, LayoutLM families were developed to enhance document comprehension by incorporating images, OCRed text, and pre-training with an awareness of the layout structure. 
However, they necessitate transfer learning for each downstream task, resulting in high model training and operation costs.
To overcome this limitation, we propose a new LayoutLLM model, which seamlessly integrates LayoutLM and large-scale language models (LLM) to improve document image understanding. 
By leveraging the strengths of LayoutLM in visual document layout comprehension and LLM's superior language comprehension capabilities, the proposed model fine-tunes a multimodal instruction data set to create a holistic understanding of document images. 
Our experiments have demonstrated significant improvement over the baseline model in various document analysis tasks, such as form understanding, receipt recognition, and invoice comprehension.

